End-to-end Learning of a Fisher Vector Encoding for Part Features in Fine-grained Recognition

Part-based approaches for fine-grained recognition do not show the expected performance gain over global methods, although explicitly focusing on small details that are relevant for distinguishing highly similar classes. We assume that part-based methods suffer from a missing representation of local features, which is invariant to the order of parts and can handle a varying number of visible parts appropriately. The order of parts is artificial and often only given by ground-truth annotations, whereas viewpoint variations and occlusions result in not observable parts. Therefore, we propose integrating a Fisher vector encoding of part features into convolutional neural networks. The parameters for this encoding are estimated by an online EM algorithm jointly with those of the neural network and are more precise than the estimates of previous works. Our approach improves state-of-the-art accuracies for three bird species classification datasets.

==> sections/01_old_intro.tex <==
%!TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

Part- or attention-based approaches~\cite{Fu_2017_CVPR,ge2019weakly,he2019and,zhang2019unsupervised,zhang2019learning,zheng2017learning} are common choices for fine-grained visual categorization (FGVC) because they explicitly focus on small details that are relevant for distinguishing highly similar classes, e.g., different bird species.
Quite surprisingly, methods that perform the categorization with global image features~\cite{Cui_2018_CVPR_large,lin2015bilinear,Simon17_GOP,Simon19:Implicit,touvron2019fixing,zheng2019learning} also achieve excellent results and it is hard to tell from the empirical results reported in the literature which general approach (global or part-based) is superior, given that all of them show comparable results in terms of recognition performance.
We hypothesize that part-based algorithms are currently not able to exploit their full potential due to the problems that arise from the initial detection of parts, especially regarding a unified representation of individual part features after the detection.
Since learning individual part detectors requires part annotations and thus additional, time-consuming efforts by domain experts, methods for unsupervised part detection have been developed that already obtain remarkable classification results~\cite{ge2019weakly,Korsch19_CSPARTS,zhang2019learning}.
However, unsupervised part detection faces various challenges, such as missing parts caused by different types of occlusions and parts with ambiguous semantic meaning, as shown in Fig.~\ref{fig:teaser}.
Hence, it remains unclear whether detected parts are reasonable and semantically consistent.
Furthermore, part-based classifiers usually require both a fixed number of parts to be determined for each image and a pre-defined order of the extracted part features, which are then handed to the classifier.
These are strong restrictions for the application, especially when considering varying poses and viewpoints that lead to hidden parts not visible in an image.
In general, we believe that a common way for representing a \emph{varying number of unordered part features} obtained from each single image is missing.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{figures/teaser}
	\caption{Comparison of traditional part feature aggregation with our proposed method based on Fisher vector encoding. In the traditional case, the problem of missing features may occur when some parts can not be detected but the resulting gaps need to be filled for the feature concatenation. Furthermore, the semantics of extracted features is not clear due to unsupervised part detection algorithms that may not preserve a consistent order of part features. With our approach, we are able to compute a unified representation of fixed length for an arbitrary number of unordered part features. This representation can then be used by any type of classifier, including simple linear classifiers and fully-connected layers in a deep neural network.}
	\label{fig:teaser}
\end{figure}


We therefore propose the integration of a well-known feature transformation method typically applied to local descriptors of keypoints, namely the Fisher vector encoding (FVE)~\cite{perronnin2007fisher,Perronnin10:ITF}, into a convolutional neural network (CNN).
The FVE enables handling different numbers of parts for each image, e.g., only those that are visible given the actual pose of the bird and the viewpoint, by computing a unified representation of fixed length independent of the number of detected parts (Fig.~\ref{fig:teaser}).
Note that the problem of missing parts can also be observed when considering the ground-truth annotations of widely-used fine-grained datasets for bird species categorization~\cite{Birdsnap,NABirds,CUB_200_2011}, which are often used to evaluate the performance of new classification algorithms without taking the part detection into account.
Common methods for filling the gaps of missing parts are simple, like the insertion of a constant value, e.g., filling with zeros~\cite{Goering14:NPT,liu2013bird,zhang2014part}.
Other strategies insert the whole input image as a part (which is then rather a global feature than a local one), or a cropped part of the image around its center point.
The latter can be motivated by a spatial prior, i.e., objects are more often located in the center of an image.
Our method does not require any gap-filling strategy.
Furthermore, it allows for neglecting an artificial order of parts since there is usually no natural order of parts and each part should be treated equally.

In contrast to previous approaches that apply different kinds of FVE together with CNNs~\cite{cimpoi2015deep,song2017locally,wieschollek2017backpropagation,tang2018deep,zhang2016picking,arandjelovic2016netvlad,gong2014vlad_pooling}, our method determines the underlying Gaussian mixture model~(GMM) with an iterative EM algorithm using mini-batch updates of parameters.
These parameters are estimated jointly with the parameters of the CNN in an end-to-end manner.
Consequently, the GMM has a direct influence on the feature extraction within the CNN and also adapts to the changing feature representations during learning.
We describe the details of our approach in Sect.~\ref{sec:methods}, which achieves new state-of-the-art accuracies for fine-grained bird species categorization on three datasets: CUB-200-2011\cite{CUB_200_2011} (improvement from 90.3\% to 91.1\%), NA-Birds\cite{NABirds} (from 89.2\% to 90.3\%), and Birdsnap\cite{Birdsnap} (from 84.3\% to 84.9\%).


==> sections/04_results/00_n_components.tex <==
%!TEX root = ../../main.tex

\begin{table}[t]
	\caption{Comparison of the number of components chosen for the Gaussian mixture model (\textbf{bold}~=~best result).}
	\begin{center}
		\begin{tabular}{lcrl}
			\toprule

			 \scriptsize{} &
			 \scriptsize{\# components} &
			 \scriptsize{Accuracy } &
			 \scriptsize{StdDev} \\
			\midrule
			GA Pooling & 	-- 	& 	91.10 & \scriptsize{$\pm 0.06$} \\
			\midrule
			FVE 		&	1  	& 	\textbf{91.45} & \scriptsize{$\pm 0.10$} \\
			FVE 		&	2  	& 	91.37 & \scriptsize{$\pm 0.11$} \\
			FVE 		&	3  	& 	91.33 & \scriptsize{$\pm 0.12$} \\
			FVE 		&	4  	& 	91.35 & \scriptsize{$\pm 0.09$} \\
			FVE 		&	5  	& 	91.29 & \scriptsize{$\pm 0.11$} \\
			FVE 		&	6  	& 	91.33 & \scriptsize{$\pm 0.18$} \\
			FVE 		&	10 	& 	91.40 & \scriptsize{$\pm 0.11$} \\
			FVE 		&	20 	& 	91.41 & \scriptsize{$\pm 0.16$} \\
			FVE 		&	50 	& 	91.44 & \scriptsize{$\pm 0.08$} \\
			\bottomrule
		\end{tabular}
	\label{tab:n_components}
	\end{center}
\end{table}


==> sections/04_results/01_order_visibility.tex <==
%!TEX root = ../../main.tex

\begin{table}[t]
\caption{Comparison of our proposed FVE with global average pooling (GAP) regarding order and visibility of parts.}
\begin{center}
\begin{tabular}{l@{\hspace{2em}}l@{\hspace{4em}}r}
	\toprule
		\small{\textsc{Method}} &
		\small{\textsc{Setup}} &
		% \small{Only visible} &
		\small{\textsc{Accuracy (std)}
		} \\
	\midrule
		% \multicolumn{2}{l}{No Parts} & & & \\
		GAP  &  \small{baseline with no parts} & 89.54 \small{$(\pm 0.15)$} \\
		% & Baseline FVE  & -- & -- & 89.91 \small{$(\pm 0.25)$} \\
	\midrule
		% \multicolumn{2}{l}{GT Parts} & & & \\
		GAP & \small{shuffled GT parts} & 90.01 \small{$(\pm 0.18)$}  \\
		FVE (ours) & \small{shuffled GT parts} & 90.56 \small{$(\pm 0.15)$}  \\
		FVE (ours) & \small{only visible GT parts} & 90.51 \small{$(\pm 0.21)$}  \\
	\midrule
		GAP  & \small{ordered GT parts} & 90.53 \small{$(\pm 0.30)$} \\
		FVE (ours) & \small{ordered GT parts} & 90.49 \small{$(\pm 0.18)$} \\
	\bottomrule
	\end{tabular}
	\label{tab:order_visibility}
	\end{center}
\end{table}




==> sections/04_results/02_joint_training.tex <==
%!TEX root = ../../main.tex
\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\textwidth]{figures/line-plot.pdf}
	\caption{Comparison of the conventional pipeline with our proposed joint learning approach described in Sect.~3 of our paper.}
	\label{fig:joint_training}
\end{figure}


==> sections/04_results/04_n_dims_comps.tex <==
%!TEX root = ../../supplement.tex

\begin{figure}[t]
	\begin{center}
	\begin{subfigure}[t]{0.48\textwidth}
		\includegraphics[width=\linewidth]{figures/n_comps}
		\caption{The EM-based method is more robust for a different number of mixture components. The gradient-based method performs worse for more than \num{16} components.}
		\label{fig:n_comps}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.48\textwidth}
		\includegraphics[width=\linewidth]{figures/n_dims}
		\caption{The gradient-based method outperforms the EM-based if dimensionality reduction is performed. Nevertheless, the higher the input dimension, the closer the EM-based method gets to the gradient-based method. Finally, we observed the best performance if no dimensionality reduction is performed ($D=2048$).}
		\label{fig:n_dims}
	\end{subfigure}
	\caption{Accuracies on the CUB-200-2011 dataset for experiments investigating the effect of the number and the dimension of the Gaussian mixture components for two different parameter estimation methods: online EM-based and gradient-based.}
	\label{fig:n_comps_dims}
	\end{center}
\end{figure}


\endinput


==> sections/04_results/05_runtime.tex <==
%!TEX root = ../../main.tex

\begin{table}[t]
\caption{Computation times for our proposed FVE-Layer.}
\begin{center}
	\begin{tabular}{@{\hspace{0.5em}}l@{\hspace{2em}}c@{\hspace{2em}}c@{\hspace{0.5em}}}
		\toprule
			\small{\textsc{Algorithm}} &
			\small{\textsc{Runtime per iteration}} &
			\small{\textsc{Relative time}} \\
		\midrule
			Overall model execution & $270.0$ ms & \pcent{100.00} \\
			Updating the GMM parameters & \phantom{27}$3.0$ ms & \phantom{10}\pcent{1.11} \\
			Computing the FVE & \phantom{27}$9.5$ ms & \phantom{10}\pcent{3.52} \\
		\bottomrule
		\end{tabular}
		\label{tab:runtime}
\end{center}
\end{table}
\endinput

Runtime for model call: 735.724sec for 2725 iterations, 270ms / iteration.
Runtime for the encoding: 25.902sec for 2725 iterations, 9.5ms / iteration.
Runtime for the EM parameter updates: 8.144sec for 2725 iterations, 3ms / iteration.

